Improving Efficiency in Large-Scale Decentralized Distributed Training

Decentralized Parallel SGD (D-PSGD) and its asynchronous variant Asynchronous Parallel SGD (AD-PSGD) is a family of distributed learning algorithms that have been demonstrated to perform well for large-scale deep learning tasks. One drawback of (A)D-PSGD is that the spectral gap of the mixing matrix decreases when the number of learners in the system increases, which hampers convergence. In this paper, we investigate techniques to accelerate (A)D-PSGD based training by improving the spectral gap while minimizing the communication cost. We demonstrate the effectiveness of our proposed techniques by running experiments on the 2000-hour Switchboard speech recognition task and the ImageNet computer vision task. On an IBM P9 supercomputer, our system is able to train an LSTM acoustic model in 2.28 hours with 7.5% WER on the Hub5-2000 Switchboard (SWB) test set and 13.3% WER on the CallHome (CH) test set using 64 V100 GPUs and in 1.98 hours with 7.7% WER on SWB and 13.3% WER on CH using 128 V100 GPUs, the fastest training time reported to date.

==> Makefile <==
.SUFFIXES: .eps .pdf
LATEX=./colourlatex.sh pdflatex
BIBTEX=bibtex
FIG2DEV=fig2dev

MAIN=main
#SUP=supplementary
#BIBMAIN=acmsmall-sample-bibfile
BIBMAIN=refs

all: $(MAIN).pdf #$(SUP).pdf #$(MAIN).ps

#FIGSEPS=$(shell ls -1 figs/*.eps)

#RESULTSEPS=$(shell ls -1 results/*.eps)

#EPS=$(FIGSEPS) $(RESULTSEPS)




MAINTEX=$(MAIN).tex \
    $(BIBMAIN).bib \

$(MAIN).pdf: $(MAINTEX) $(EPS) $(BIBMAIN).bbl
	@echo Compiling $(MAIN)
	@$(LATEX) $(MAIN)
	@$(MAKE) fixlabels

# SUPTEX=$(SUP).tex \
#     $(BIBMAIN).bib \

# $(SUP).pdf: $(SUPTEX) $(EPS) $(BIBMAIN).bbl
# 	@echo Compiling $(SUP)
# 	@$(LATEX) $(SUP)
# 	@$(MAKE) fixlabels
 

# $(MAIN).pdf: $(MAIN).dvi
# 	@dvipdfmx -p letter $(MAIN).dvi

# $(MAIN).ps: $(MAIN).dvi
# 	@dvips $(MAIN).dvi
# 	@pkill -HUP -f "^gv .*$@" || true


fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' $(MAIN).log),0)
	@echo $(MAIN) Compiling again to fix labels
	@$(LATEX) $(MAIN)
else
	@echo $(MAIN) Labels are correct
endif

$(BIBMAIN).bbl: $(BIBMAIN).bib
	@echo Compiling required EPS files
	#@make -C figs
	@echo Compiling main for bibliography
	@$(LATEX) $(MAIN)
	@echo Generating bibliography
	@$(BIBTEX) $(MAIN)
	@echo Recompiling main after generating bibliography
	@$(LATEX)  $(MAIN)
	@$(MAKE) fixlabels
	# @echo Compiling SUP for bibliography
	# @$(LATEX) $(SUP)
	# @echo Generating bibliography
	# @$(BIBTEX) $(SUP)
	# @echo Recompiling SUP after generating bibliography
	# @$(LATEX)  $(SUP)
	# @$(MAKE) fixlabels

%.eps.pdf: %.eps
	@echo "	" Converting $< to $(@)
	@epstopdf --outfile=figs/$(@) $<

clean:
	#@make -C figs clean
	@/bin/rm -f $(MAIN).ps $(MAIN).pdf *.aux *.dvi *.log *.bbl *.blg figs/*.pdf figures/plot/*.pdf *.toc *.out *.bak


==> analysis.tex <==
\section{Analysis}

\begin{table*}
\begin{tabular}{|l|l|l|l|l|}
\hline
         & Spectral-Gap & Connectivity Degree & Comm-Traffic-Per-Learner & Global Barrier \\ \hline
D-PSGD   & x            & 2                   & 2*$\vert M\vert$                    & N              \\ \hline
RAD-PSGD & x            & 2                   & 2*$\vert M\vert$                    & N              \\ \hline
D1       & 0            & N                   & N*$\vert M\vert$                    & Y              \\ \hline
\end{tabular}
\caption{Traffic Analysis}
\label{tab:traffic-analysis}
\end{table*}


==> dl_speedup.tex <==
Consider the following stochastic optimization problem
\begin{align}
      \min_{\theta} F(\theta) =  \mathbb{E}_{\xi}[f(\theta;\xi)]
\end{align}
where $F$ is the objective function, $\theta$ is the parameters to be optimized (it is the weights of networks for DL) and $\xi\!\sim\!p(x)$ is a random variable on the training data $x$ obeying distribution $p(x)$. Supposing that there are $n$ training samples and $\xi$ assumes a uniform distribution,  $\xi\!\sim\!\text{Uniform}\{1, \cdots, n\}$,  we have
\begin{align}
      \min_{\theta} F(\theta) =  \mathbb{E}_{\xi}[f(\theta;\xi)] = \frac{1}{n}\sum_{i=1}^{n}f_{i}(\theta)
\end{align}
where $f_{i}(\theta)$ is evaluated at training sample $x_{i}$. In mini-batch based SGD, at each iteration $k$, we have
\begin{align}
      F(\theta_{k+1}) = F(\theta_{k}) - \alpha_{k}g(\theta_{k},\xi_{k})
\end{align}
where $\alpha_{k}$ is the learning rate and
\begin{align}
    g(\theta_{k},\xi_{k}) \triangleq \frac{1}{m}\sum_{s=1}^{m}\nabla f(\theta_{k},\xi_{k,s})
\end{align}
with $m$ being the size of the mini-batch.


\begin{figure}[t]
  \centering{
        \includegraphics[width=0.40\textwidth]{figures/decentr-networks_v2-crop.pdf}
  }
  %\vspace{-1em}
  \caption{A centralized distributed learning architecture (aka Parameter-Server architecture) and a decentralized distributed learning architecture}
  \label{fig:decen-graphs}
  %\vspace{-1em}
\end{figure}

DL problem is an optimization problem described above. DDL is the distributed computing paradigm that solves DL problems. At the dawn of DDL research, the Parameter Server (PS) architecture \cite{distbelief} was wildy popular. \Cref{fig:decen-graphs}(a) illustrates a PS design: each learner calculates gradients and sends them to the PS, before the PS sends the updated weights back to the learners.
The core of PS architecture is the ASGD algorithm that allows each learner to calculate gradients and asynchronously push/pull the gradients/weights to/from the PS. The weight update rule in ASGD is given in \Cref{eqn:update_async}:{
\begin{align}
    F(\theta_{k+1}) & = F(\theta_{k}) - \alpha_{k} g(\theta^{\zeta_{i}}_{k},\xi^{\zeta_{i}}_{k})  \label{eqn:update_async}
\end{align}
where $\zeta_{i} \in \{1, \cdots, \lambda\}$ is an indicator of the learner which made the model update at iteration $k$.
Soon researchers realized that such design led to sub-par models that can be trained fast but accuracy-wise significantly lag behind single-learner baseline because of the large system staleness issue \cite{zhang-ijcai-2016, revisit-sync-sgd, zhang2016icdm}.
SSGD regained its popularity mainly because the synchronization problems exacerbated by the cheap commodity systems could be addressed by decades of High Performance Computing (HPC) research. In SSGD, the weight update rule is given in \Cref{eqn:update_sync}
: each learner calculates gradients and receives updated weights in lockstep with the others.\footnote{Throughout this paper, we use $\lambda$ to denote the number of learners.} SSGD has exactly the same convergence rate as the single learner baseline while enjoying reasonable speedup. %% The weights used to calculate the gradients are always the same as the one on the PS, thus staleness is 0.

\begin{align}
    F(\theta_{k+1}) & = F(\theta_{k}) - \alpha_{k}\left[\frac{1}{\lambda}\sum_{i=1}^{\lambda} g(\theta^{i}_{k},\xi^{i}_{k})\right] \label{eqn:update_sync}
\end{align}

The summation and the following broadcast in \Cref{eqn:update_sync} is known as the ``All-Reduce'' operation in the HPC, which is a well-studied operation. When the message to be ``AllReduced'' is large, as in the DL case, an optimal algorithm exists that maximizes the communication bandwidth utilization \cite{fsu-allreduce}. Many incarnations of this algorithm exist, such as \cite{paddle-paddle,nccl,ddl}.
Like any synchronous algorithm, SSGD is subject to the \textit{straggler problem}, which means a slow learner slows down the entire training system.

Wildfire \cite{wildfire} is the first decentralized training system that has been demonstrated to work on modern deep learning tasks. The follow-up work in \cite{dpsgd, adpsgd} rigorously proved the decentralized parallel SGD algorithm in both synchronous and asynchronous forms can maintain the SSGD convergence rate while resolving the straggler problem. \Cref{fig:decen-graphs}(b) illustrates a decentralized parallel SGD system , where each learner $i$ calculates the gradients, updates its weights, and averages its weights with its neighbor $j$ in a ring topology. DPSGD/ADPSGD weights update rule is defined in \Cref{eqn:update_decentr}.

\begin{align}
    \Theta_{k+1} = \Theta_{k}T_{k} - \alpha_{k} g(\Theta_{k},\bm{\Xi}_{k})  \label{eqn:update_decentr}
\end{align}
where the columns of $\Theta_{k} = [\theta^{1}_{k}, \cdots, \theta^{\lambda}_{k}]$ are the weights of each learner; the columns of $\Xi_{k} = [\xi^{1}_{k}, \cdots, \xi^{\lambda}_{k}]$ are random variables associated with batch samples; the columns of $g(\Theta_{k},\bm{\Xi}_{k})  = [g(\theta^{1}_{k},\xi^{1}_{k}), \cdots, g(\theta^{\lambda}_{k},\xi^{\lambda}_{k})]$ are the gradients of each learner, and $T_{k}$ is a symmetric stochastic matrix (therefore doubly stochastic) with two $0.5$s at neighboring positions for each row and column and 0s everywhere else. This amounts to performing model averaging with one learner's left or right neighbor in the ring for each mini-batch weights update. The key difference between \dpsgd and \adpsgd is that \adpsgd allows overlapping of gradients calculation and weights averaging and removes the global barrier in \dpsgd that forces every learner to synchronize at the end of each minibatch training. Naturally, \adpsgd runs much faster than \dpsgd.



==> motivation.tex <==
\section{Motivation}
\sg increases when number of learners is getting bigger.
\begin{figure}[t]%[!htpb]
\small
    \centering
    \subfloat[{ImageNet accuracy}]{{ \includegraphics[width=0.24\textwidth, scale=0.6]{./figures/imagenet_motivation} }\label{fig:corr_jewel}}%\hfill
    \subfloat[{\swbb Held-out loss}]{{ \includegraphics[width=0.24\textwidth, scale=0.6]{./figures/swb2000_motivation} }\label{fig:corr_welltok}}%\hfill
    
\caption{motivation}
    \label{fig:correctness_gadei}
\end{figure}

